Batch DropBlock Network for Person Re-identification and Beyond

Since the person re-identification task often suffers from the problem of pose changes and occlusions, some attentive local features are often suppressed when training CNNs. In this paper, we propose the Batch DropBlock (BDB) Network which is a two branch network composed of a conventional ResNet-50 as the global branch and a feature dropping branch. The global branch encodes the global salient representations. Meanwhile, the feature dropping branch consists of an attentive feature learning module called Batch DropBlock, which randomly drops the same region of all input feature maps in a batch to reinforce the attentive feature learning of local regions. The network then concatenates features from both branches and provides a more comprehensive and spatially distributed feature representation. Albeit simple, our method achieves state-of-the-art on person re-identification and it is also applicable to general metric learning tasks. For instance, we achieve 76.4% Rank-1 accuracy on the CUHK03-Detect dataset and 83.0% Recall-1 score on the Stanford Online Products dataset, outperforming the existing works by a large margin (more than 6%).

==> problem.tex <==
\section{Problem Formulation}
Person re-identification is often formulated as an image retrieval problem, which aims to find the most similar image from a large set of candidate images. This retrieval problem can be solved by finding an embedding function $f(\cdot)$ and a metric function $D(\cdot, \cdot)$, where the embedding maps an input image $x$ to a high dimensional feature vector $f(x)$ and the metric $D(f(x), f(y))$ measures the similarity between two embedding vectors $f(x)$ and $f(y)$. 
In this paper, we simply take the Euclidean distance  as the metric $D(\cdot, \cdot)$ and seek to train a neural network to learn the embedding $f(\cdot)$. 
We formulate the general image retrieval problem as the following.
Given a dataset $\mathcal{X}$ with $C$ classes, we split it into the training set $\mathcal{X}_{train}$ and testing set $\mathcal{X}_{test}$ with $C_{train}$ and  $C_{test}$  classes respectively. Notice that there is no overlap between $C_{train}$ and $C_{test}$. We train the network to learn the embedding $f(\cdot)$ with appropriate loss functions from image batches sampled in $\mathcal{X}_{train}$. 
During testing, we first compute the feature embedding for all images in $\mathcal{X}_{test}$ to build a database of embedding vectors $\mathcal{F}_{test}$. Then for each test image $q$ in $\mathcal{X}_{test}$, we compute its embedding $f_q$ and search the $K$ nearest neighbors (KNN) in the embedding database $\mathcal{F}_{test}$. The embedding of the query image itself is excluded from these $K$ nearest neighbors. For each returned KNN result, we consider it is correct if its class is the same as the query image's class.

Person re-ID can be regarded as image retrieval where each person corresponds to a class. Person re-ID can be regarded as image retrieval where each person  corresponds to a class. In addition, each person image has a camera ID indicating the camera it is captured from. In person re-ID, challenging query images are selected for each person in the testing set $\mathcal{X}_{test}$ to form the query dataset $\mathcal{X}_{query}$. The gallery dataset $\mathcal{X}_{gallery}$ consists of the remaining testing images. In other words, a person re-ID dataset $\mathcal{X}$ is split to $\mathcal{X}_{train}$, $\mathcal{X}_{query}$, and $\mathcal{X}_{gallery}$. The training set $\mathcal{X}_{train}$ contains $C_{train}$ identities, while $\mathcal{X}_{query}$ and $\mathcal{X}_{gallery}$ contain the same $C_{test}$ identities. The training process of our person re-ID is exactly the same as general image retrieval. During testing, we compute the embedding database $\mathcal{F}_{gallery}$ for gallery dataset and query KNN results for each query image in $\mathcal{X}_{query}$. To make the problem more challenging, we only consider a result is correct when it has the same person identity and different camera ID from the query image.

In addition, each person image has a camera ID indicating the camera it is captured from. In person re-ID, challenging query images are selected for each person in the testing set $\mathcal{X}_{test}$ to form the query dataset $\mathcal{X}_{query}$. The gallery dataset $\mathcal{X}_{gallery}$ consists of the remaining testing images. In other words, a person re-ID dataset $\mathcal{X}$ is split to $\mathcal{X}_{train}$, $\mathcal{X}_{query}$, and $\mathcal{X}_{gallery}$. The training set $\mathcal{X}_{train}$ contains $C_{train}$ identities, while $\mathcal{X}_{query}$ and $\mathcal{X}_{gallery}$ contain the same $C_{test}$ identities. The training process of our person re-ID is exactly the same as general image retrieval. During testing, we compute the embedding database $\mathcal{F}_{gallery}$ for gallery dataset and query KNN results for each query image in $\mathcal{X}_{query}$. To make the problem more challenging, we only consider a result is correct when it has the same person identity and different camera ID from the query image.

